DAGGER: A Scalable Index for Reachability Queries in Large Dynamic Graphs

With the ubiquity of large-scale graph data in a variety of application domains, querying them effectively is a challenge. In particular, reachability queries are becoming increasingly important, especially for containment, subsumption, and connectivity checks. Whereas many methods have been proposed for static graph reachability, many real-world graphs are constantly evolving, which calls for dynamic indexing. In this paper, we present a fully dynamic reachability index over dynamic graphs. Our method, called DAGGER, is a light-weight index based on interval labeling, that scales to million node graphs and beyond. Our extensive experimental evaluation on real-world and synthetic graphs confirms its effectiveness over baseline methods.

==> experiments_shortenedBackup.tex <==
\section{Experiments}

In this section, we evaluate the effectiveness of DAGGER on various
real and synthetic datasets. We compare DAGGER with 
the baseline Depth-First
Search (DFS).
The other methods are not included in our comparison 
because of the following issues with them:
i) Optimal-Tree Cover~\cite{agrawal}: Although it mentions
how to update the index for some operations, it does not support
all operations. Furthermore, it assumes the graph is always acyclic.
ii) Incremental-2HOP~\cite{bramandiaJ}: The existing
implementation do not support all update operations. It
supports edge insertions and node deletions.
iii) \cite{krommidas2008} provides an experimental analysis 
and implementations of the dynamic transitive closure
\cite{roditty,king-jcss02,king,henzinger,demetrescu2000}
approaches. However,
none of them are scalable as they require quadratic space.  

In these experiments, we attempt to index very large dynamic
graphs on a system with a quad-core Intel i5-2520M 2.50Ghz
processor, with
4GB memory. To the best of our knowledge, the largest 
dynamic graphs previously used for reachability queries had 
400K nodes~\cite{bramandiaJ}.
Furthermore, that study only applied node deletions.
In that sense, our 
study is unique in that it scales to million node graphs, and
includes a comprehensive evaluation over an intermixed sequence
of update operations, i.e., our evaluation includes all four
update operations -- edge/node insertion/deletion. 


\subsection{Experimental Setup}
To effectively and realistically
evaluate the cost of index maintenance, we intersperse
reachability queries with the graph update operations.
We then compare \alg with DFS to find out
under which conditions \alg's fast querying 
amortizes the maintenance cost of the index.
Note that DFS has no update cost, but pays a penalty in terms of  longer query 
times. Thus, in a scenario that receives queries
very rarely (e.g., 1 query per hundreds of updates),
it is obvious that maintaining an index would not pay
off. Thus, in our experiments we vary the ratio of queries
to update operations, and measure the total time which
includes the query and update times for both DFS and \alg.
For each dataset, we report the average time for the update
operations and queries, as well as the
total time taken for $q$ queries per update (QpU), 
where $q$ ranges from one to eight.  As we shall see, \alg
typically outperforms DFS after just 2 queries per update, with
the gap increasing as this ratio goes up. This 
makes it an effective index for dynamic real-world graph querying.

\begin{table}
\centering
\scalebox{0.8}{
 \begin{tabular}{ll|r|r|r|r}
\multicolumn{2}{c|}{Graph} & Node & Edge & DAG & Largest \\
\multicolumn{2}{c|}{Dataset} & Size & Size & Size & SCC\\
\hline
\multirow{2}{*}{FrenchWiki} &Initial & 999,447 & 3,452,667 & 899,343  &  97,465\\
& Final & 999,499 & 3,452,953 & 899,360 & 97,502 \\
\hline
\multirow{2}{*}{PatentCitation}& Initial & 605,617 & 1,000,002 & 605,617  &  1\\
& Final & 705,617 & 1,205,190 & 705,617 & 1 \\
\hline
\multirow{2}{*}{ER1M}& Initial & 1,000,000 &1,500,123 & 659,892 & 340,109\\
& Final & 1,000,170 & 1,500,631 & 659,647 & 340,505 \\
\hline
\multirow{2}{*}{BA1M}& Initial & 1,000,000 &2,000,823 &  478,219 & 521,782 \\
& Final & 1,000,182 & 2,001,313 & 478,240 & 521,930
\end{tabular}
}
\vspace{-0.1in}
\caption{\small Properties of dynamic datasets: Node size refers
to $|V^i|$, edge size to $|E^i|$, and DAG to $|V^d|$; Largest SCC
refers the component $size$, i.e., number of nodes in the largest SCC.}
\label{tab:dynamicdata}
\end{table}

\subsection{Datasets}

As opposed to the static setting, evaluation of dynamic indexing
requires a valid sequence of update operations, as well as the
queries, along with an initial graph. We used both real and
synthetic graph datasets in our experiments, as shown in
Table~\ref{tab:dynamicdata}.  The row marked ``Initial'' shows
the properties of the input graphs, whereas the row marked
``Final'' shows the same properties after the completion of all
the update operations.

\smallskip\noindent
\textbf{Real Graph Evolution: } For these datasets we were
able to compile the complete evolution of a graph at the edge
level. We have two such datasets:
\begin{list}{\labelitemi}{\leftmargin=1em}
 \item {FrenchWiki}: Wikimedia Foundation dumps the snapshots
	 of Wikipedia in certain intervals (see
	 \url{dumps.wikimedia.org}).
These dumps contain all the textual content with full
revision/edit history. We discarded the textual content
and recovered the evolution of the complete French language Wikipedia graph from
its birth by comparing the consecutive versions of
each page. If a new wiki-link is added in a version
of a wiki-page, we consider it as an insertion of
an edge with the timestamp of that version of the wiki-page. 
Similarly, if an existing wiki-link disappears in a version
of a wiki-page, we consider it as an edge deletion.
We took a snapshot of the graph and indexed it
when it had 1 million nodes, and we then applied the next 1000
update operations to the indexed graph.
\item {PatentCitation}: This graph 
includes all citations 
within patents granted in the US between 1975 and 1999 (see
\url{snap.stanford.edu/data/cit-Patents.html}). Since
the timestamps of the patents are also available, so we can simulate
the growth of the data. Note that the only update in this data is 
node additions with a set of outgoing edges. Therefore it is 
always an acyclic graph. We indexed a snapshot
of the graph when it had around 600K nodes, and we then 
applied the following 100,000 node additions
to the initial graph as update operations.
\end{list}

\smallskip\noindent
\textbf{Synthetic Graph Evolution: } For these datasets, we first
generated three different random graphs. 
We then generated a synthetic
update sequence of 1,000 operations. Our random graphs are:
\begin{list}{\labelitemi}{\leftmargin=1em}
\item {ER1M}: We generated a directed graph of 1 million nodes, and
	1.5 million edges using the Erdos-Renyi (ER)~\cite{ER} random
	graph model.  Each edge is selected by choosing a source and
	a target node, both uniformly at random, and directing the
	edge from the source to the target.
\item {BA1M}: The Barabasi-Albert (BA) preferential
	attachment model~\cite{Barabasi1999} is a generative model
	which retains some real-world graph properties such as
	power-law degree distributions. The average degree $d$ is a
	parameter of the model. Starting from $2d$ initial nodes, at
	each time step a new node is added to the graph, with some
	outgoing edges to the existing nodes. The number of outgoing
	edges is chosen randomly in the range [1,2d]. Further, the
	end point for each edge is ``preferentially'' selected with
	probability proportional to the degree of the existing node.
	In other words, when node $w$ is being inserted, it will be
	connected to node $x$ via the edge $(w,x)$ with probability
	$degree(x)/2m$ where $m$ is the current edge size of the
	graph. To obtain possibly cyclic graphs with BA model, we
	reversed the new edges with probability $0.5$. Therefore, the
	generative BA process can create cycles. 
	We generated a graph with 1 million nodes using this directed
	BA model (with $d=2$).
\end{list}

For each of the synthetic graphs, we randomly generated update
sequences using a preferential attachment model.  In the
generation of the update sequence, we first select the operation
type with predefined ratios (for instance, we used 60\% insert
edge, 15\% delete edge, 20\% insert node, 5\% delete node, which
can be considered as representing a insertion focused graph
growth scenario, with more weight on adding edges).
Since we also report the average time for each operation, 
the exact
ratios of different operations does not effect our conclusions.
The sequence of update operations is generated as follows:
\begin{itemize}
 \item Insert Edge: Select source node uniformly at random and target
node via preferential attachment.
 \item Delete Edge: Select an edge from the existing edges uniformly at random.
 \item Insert Node: Randomly determine the indegree and outdegree of the
node, then select the other ends for these edges via preferential 
attachment.
 \item Delete Node: Select a node uniformly at random and delete
it with its incident edges.
\end{itemize}
 
In our experiments, we measure the average update times (i.e.,
edge insertion time (EI), node insertion time (NI), edge deletion
time (ED) and node deletion time (ND)) during the lifetime of a
dynamic reachability index. We used three versions of \alg --
DG0, DG1 and DG2 correspond to \alg with no intervals ($k=0$), 1
interval ($k=1$), and 2 intervals ($k=2$) per node, respectively.
Note that DG0 maintains only the DAG graph without using any
interval labeling and answers queries by performing a search on
the DAG graph. In contrast, the basic DFS performs the query
directly on the input graph, since it obviously does not maintain
the DAG.


\begin{figure*}[!ht]
\centerline{
\subfigure[FrenchWiki]{
\includegraphics[width=1.35in,height=1.5in]{./daggerplots/frwiki_n7550000.tt-bw.eps}	
}
\subfigure[PatentCitation]{
\includegraphics[width=1.35in,height=1.5in]{./daggerplots/cit-Patents.txt.sorted.tt-bw.eps}	
}
\subfigure[ER1M]{
\includegraphics[width=1.35in,height=1.5in]{./daggerplots/er1Mk2.tt-bw.eps}	
}
\subfigure[BA1M]{
\includegraphics[width=1.35in,height=1.5in]{./daggerplots/ba1Mk2bidir.tt-bw.eps}	
}}
\vspace{-0.15in}
\caption{\small Total time comparison on dynamic datasets}
\label{fig:dynamictotal}
\end{figure*}

\begin{table}[!ht]
\centering
\small
\subtable[Real Graphs]{
\begin{tabular}{|l||ccccc||cc|}
\hline
Data & \multicolumn{5}{|c||}{FrenchWiki} & \multicolumn{2}{|c|}{Citation}\\
\hline
Method & Q & EI & ED & NI & ND & Q & NI\\
\hline
DFS & 410 & - & - & - & - & 0.19 & - \\
DG0 & 221 & 60 & 253 & 0.06 & 191 & 0.31 & 0.06 \\
DG1 & 148 & 48 & 267 & 0.02 & 189 & 0.10 & 0.06 \\
DG2 & 128 & 62 & 279 & 0.02 & 192 & 0.08 & 0.06 \\
\hline
\end{tabular}
}
%\caption{\small Average Operation Times (in ms) on Real Data}
%\end{table}
\vspace{0.2in}
%\begin{table*}
\centering
\subtable[Synthetic Graphs]{
\begin{tabular}{|l||ccccc|}
\hline
Data & \multicolumn{5}{|c|}{ER1M}\\
\hline
Method & Q & EI & ED & NI & ND\\
\hline
DFS & 311 & - & - & - & -  \\
DG0 & 119 & 212 & 775 & 0.01 & 538\\
DG1 & 46 & 203 & 832 & 0.13 & 548\\
DG2 & 44 & 319 & 871 & 0.10 & 562\\
\hline
\multicolumn{6}{|c|}{~}\\
\hline
Data & \multicolumn{5}{|c|}{BA1M}\\
\hline
Method & Q & EI & ED & NI & ND\\
\hline
DFS & 448 & - & - & - & - \\
DG0 & 75 & 172 & 2032 & 0.03 & 2726 \\
DG1 & 39 & 148 & 2138 & 0.13 & 2769  \\
DG2 & 38 & 218 & 2202 & 0.07 & 2804 \\
\hline
\end{tabular}
}
\vspace{-0.3in}
\caption{\small Average Operation Times (in ms) on Real and
Synthetic Data. $Q$ refers to query time, $EI$ and $ED$ to edge
insertion and deletion, and $NI$ and $ND$ to node insertion and
deletion.}
\vspace{-0.2in}
\label{tab:dynamicresults}
\end{table}

\subsection{Results}

In Figure~\ref{fig:dynamictotal}, we plot the total time taken to
perform all the operations (updates and queries) for DFS and 
the \alg variants DG0,
DG1, and DG2. The total time (in sec) is plotted against the
number of reachability queries per update operation. DAGGER has the
advantage of fast querying at the cost of index maintenance,
whereas DFS has no update cost. These plots make it clear that 
DG1 amortizes the maintenance costs as long as there are 
2-4 queries per update operation, which is quite reasonable
for an online system. The average update and query times on 
each of the graph datasets are shown in
Tables~{\ref{tab:dynamicresults}(a)} and {\ref{tab:dynamicresults}(b)}.
We discuss dataset specific results below.

\textbf{FrenchWiki:} In Figure~\ref{fig:dynamictotal}(a),
we see that DG0 performs better DFS in total time starting with 
4 queries per update. 
In other words, the efficient dynamic DAG/SCC maintenance in \alg
is enough to outperform the baseline DFS method.
On the other hand, the interval labeling and maintenance in \alg
offers even more significant benefits.
We can observe that 
\alg with interval labeling is better than DFS after just
2 queries per update. 
However, it is interesting to note that there is no big 
difference in the performance of DG1 and DG2. That is, using two
interval labels does not improve the total time. 
In Table~{\ref{tab:dynamicresults}(a)} we can see that whereas the
average query time is indeed better for DG2, unfortunately it
incurs more overhead for the update operations due to the
extra cost of maintaining one more interval, in particular for
edge insertion/deletion.


\textbf{PatentCitation:} In this dataset the only update
operation is node insertion with outgoing edges. From
Table~{\ref{tab:dynamicresults}(a)} we observe that the cost of node
insertions are very close for all versions of DAGGER due to the
fact that there is no DAG maintenance (e.g., input graph is
always a DAG) and no label propagation. Therefore, the plot in
Figure~\ref{fig:dynamictotal}(b) reflects mainly the query time of
the methods. DG0 has worse query times than DFS, even though it
performs the same search as DFS, which can be attributed to the
overhead of the \alg graph.  However, dynamic interval labeling
provides a significant improvement on querying performance, with
two intervals (DG2) providing better query times than a single
interval label per node (DG1).

\textbf{ER1M: } Table~\ref{tab:dynamicdata} shows that this graph
has a large connected component one-third the size of the input
graph; almost all the remaining nodes are single node components.
Table~{\ref{tab:dynamicresults}(b)} shows the break down in terms of
average operation times.  We observe that DFS querying is three
times slower than even DG0! Further, dynamic interval labeling
helps, but the small query performance gain obtained by utilizing
two intervals per node instead of single interval does not pay
off the label maintenance cost. In particular, edge insertion
with DG2 is significantly slower than DG1, because when the
interval of the huge component is enlarged, this change has to be
propagated up for all the incoming edges of the huge component,
and there can be many such incoming edges.  However, the cost of
edge insertion does not increase when moving from DG0 to DG1,
because interval labels also provide pruning when updating the
DAG. The plot in Figure~\ref{fig:dynamictotal}(c) shows that DG1 is
the best method overall, and all \alg variants are preferable to
DFS, if there are at least 2 queries per update.

\textbf{BA1M: } The results are similar to those
for ER1M (see Table~{\ref{tab:dynamicresults}(b)}).
The main difference is that BA1M has a much larger SCC,
which reduces the size of the DAG significantly. Hence,
there is a greater performance difference between DFS and
\alg methods as seen in Figure~\ref{fig:dynamictotal}(e). DG1
outperforms DFS starting with 2 queries per update.

In summary, over all the real and synthetic datasets, we observe
that typically DG1 gives the best overall performance, whereas
even DG0 (i.e., just maintaining the strongly connected
components without labeling) results in a significant improvement
over DFS. 
%The cost of update operations with \alg are in the order of the
%cost of querying with DFS, therefore the index amortizes the
%maintenance cost if it receives at least a few queries per
%update operation..  
As expected, \alg amortizes the index maintenance cost against
query times, and thus the more the queries received, the more the
benefit.  It is also interesting to note that a single interval
label provides the best performance, and going to two labels does
not confer any effective advantage.  There are two reasons for
this: i) when the DAG corresponding to the input graph is very
sparse (or tree-like), a single interval is sufficient to provide
fast querying, since it captures most of the topology, and ii)
dynamically updating labels makes the labels less random, since
our current label propagation algorithm is deterministic, and of
course there is extra cost associated with label propagation.



==> experiments_shortened_hilmi.tex <==
\section{Experiments}

In this section, we evaluate the effectiveness of DAGGER on various
real and synthetic datasets. We compare DAGGER with 
the baseline Depth-First
Search (DFS).
The other methods are not included in our comparison 
because of the following issues with them:
i) Optimal-Tree Cover~\cite{agrawal}: Although it mentions
how to update the index for some operations, it does not support
all operations. Furthermore, it assumes the graph is always acyclic.
ii) Incremental-2HOP~\cite{bramandiaJ}: The existing
implementation do not support all update operations. It
supports edge insertions and node deletions.
iii) \cite{krommidas2008} provides an experimental analysis 
and implementations of the dynamic transitive closure
\cite{roditty,king-jcss02,king,henzinger,demetrescu2000}
approaches. However,
none of them are scalable as they require quadratic space.  

In these experiments, we attempt to index very large dynamic
graphs on a system with a quad-core Intel i5-2520M 2.50Ghz
processor, with
4GB memory. To the best of our knowledge, the largest 
dynamic graphs previously used for reachability queries had 
400K nodes~\cite{bramandiaJ}.
Furthermore, that study only applied node deletions.
In that sense, our 
study is unique in that it scales to million node graphs, and
includes a comprehensive evaluation over an intermixed sequence
of update operations, i.e., our evaluation includes all four
update operations -- edge/node insertion/deletion. 


\subsection{Experimental Setup}
To effectively and realistically
evaluate the cost of index maintenance, we intersperse
reachability queries with the graph update operations.
We then compare \alg with DFS to find out
under which conditions \alg's fast querying 
amortizes the maintenance cost of the index.
Note that DFS has no update cost, but pays a penalty in terms of  longer query 
times. Thus, in a scenario that receives queries
very rarely (e.g., 1 query per hundreds of updates),
it is obvious that maintaining an index would not pay
off. Thus, in our experiments we vary the ratio of queries
to update operations, and measure the total time which
includes the query and update times for both DFS and \alg.
For each dataset, we report the average time for the update
operations and queries, as well as the
total time taken for $q$ queries per update (QpU), 
where $q$ ranges from one to eight.  As we shall see, \alg
typically outperforms DFS after just 2 queries per update, with
the gap increasing as this ratio goes up. This 
makes it an effective index for dynamic real-world graph querying.

\begin{table}
\centering
\scalebox{0.8}{
 \begin{tabular}{ll|r|r|r|r}
\multicolumn{2}{c|}{Graph} & Node & Edge & DAG & Largest \\
\multicolumn{2}{c|}{Dataset} & Size & Size & Size & SCC\\
\hline
\multirow{2}{*}{FrenchWiki} &Initial & 999,447 & 3,452,667 & 899,343  &  97,465\\
& Final & 999,499 & 3,452,953 & 899,360 & 97,502 \\
\hline
\multirow{2}{*}{PatentCitation}& Initial & 605,617 & 1,000,002 & 605,617  &  1\\
& Final & 705,617 & 1,205,190 & 705,617 & 1 \\
\hline
\multirow{2}{*}{ER1M}& Initial & 1,000,000 &1,500,123 & 659,892 & 340,109\\
& Final & 1,000,170 & 1,500,631 & 659,647 & 340,505 \\
\hline
\multirow{2}{*}{BA1M}& Initial & 1,000,000 &2,000,823 &  478,219 & 521,782 \\
& Final & 1,000,182 & 2,001,313 & 478,240 & 521,930
\end{tabular}
}
\vspace{-0.1in}
\caption{\small Properties of dynamic datasets: Node size refers
to $|V^i|$, edge size to $|E^i|$, and DAG to $|V^d|$; Largest SCC
refers the component $size$, i.e., number of nodes in the largest SCC.}
\label{tab:dynamicdata}
\end{table}

\subsection{Datasets}

As opposed to the static setting, evaluation of dynamic indexing
requires a valid sequence of update operations, as well as the
queries, along with an initial graph. We used both real and
synthetic graph datasets in our experiments, as shown in
Table~\ref{tab:dynamicdata}.  The row marked ``Initial'' shows
the properties of the input graphs, whereas the row marked
``Final'' shows the same properties after the completion of all
the update operations.

\smallskip\noindent
\textbf{Real Graph Evolution: } For these datasets we were
able to compile the complete evolution of a graph at the edge
level. We have two such datasets:
\begin{list}{\labelitemi}{\leftmargin=1em}
 \item {FrenchWiki}: Wikimedia Foundation dumps the snapshots
	 of Wikipedia in certain intervals (see
	 \url{dumps.wikimedia.org}).
These dumps contain all the textual content with full
revision/edit history. We discarded the textual content
and recovered the evolution of the complete French language Wikipedia graph from
its birth by comparing the consecutive versions of
each page. If a new wiki-link is added in a version
of a wiki-page, we consider it as an insertion of
an edge with the timestamp of that version of the wiki-page. 
Similarly, if an existing wiki-link disappears in a version
of a wiki-page, we consider it as an edge deletion.
We took a snapshot of the graph and indexed it
when it had 1 million nodes, and we then applied the next 1000
update operations to the indexed graph.
\item {PatentCitation}: This graph 
includes all citations 
within patents granted in the US between 1975 and 1999 (see
\url{snap.stanford.edu/data/cit-Patents.html}). Since
the timestamps of the patents are also available, so we can simulate
the growth of the data. Note that the only update in this data is 
node additions with a set of outgoing edges. Therefore it is 
always an acyclic graph. We indexed a snapshot
of the graph when it had around 600K nodes, and we then 
applied the following 100,000 node additions
to the initial graph as update operations.
\end{list}

\smallskip\noindent
\textbf{Synthetic Graph Evolution: } For these datasets, we first
generated three different random graphs. 
We then generated a synthetic
update sequence of 1,000 operations. Our random graphs are:
\begin{list}{\labelitemi}{\leftmargin=1em}
\item {ER1M}: We generated a directed graph of 1 million nodes, and
	1.5 million edges using the Erdos-Renyi (ER)~\cite{ER} random
	graph model.  Each edge is selected by choosing a source and
	a target node, both uniformly at random, and directing the
	edge from the source to the target.
\item {BA1M}: %The Barabasi-Albert (BA) preferential
	%attachment model~\cite{Barabasi1999} is a generative model
	%which retains some real-world graph properties such as
	%power-law degree distributions. The average degree $d$ is a
	%parameter of the model. Starting from $2d$ initial nodes, at
	%each time step a new node is added to the graph, with some
	%outgoing edges to the existing nodes. The number of outgoing
	%edges is chosen randomly in the range [1,2d]. Further, the
	%end point for each edge is ``preferentially'' selected with
	%probability proportional to the degree of the existing node.
	%In other words, when node $w$ is being inserted, it will be
	%connected to node $x$ via the edge $(w,x)$ with probability
	%$degree(x)/2m$ where $m$ is the current edge size of the
	%graph. 
  The Barabasi-Albert (BA) model by definition generates acyclic graphs.
  To obtain possibly cyclic graphs with BA model, we
	reversed the new edges with probability $0.5$. %Therefore, the
	%generative BA process can create cycles. 
	We generated a graph with 1 million nodes using this directed
	BA model (with $d=2$).
\end{list}

For each of the synthetic graphs, we randomly generated update
sequences using a preferential attachment model.  In the
generation of the update sequence, we first select the operation
type with predefined ratios (for instance, we used 60\% insert
edge, 15\% delete edge, 20\% insert node, 5\% delete node, which
can be considered as representing a insertion focused graph
growth scenario, with more weight on adding edges).
Since we also report the average time for each operation, 
the exact
ratios of different operations does not effect our conclusions.
The sequence of update operations is generated as follows: 
i) Insert Edge: Select source node uniformly at random and target
node via preferential attachment.
ii) Delete Edge: Select an edge from the existing edges uniformly at random.
iii) Insert Node: Randomly determine the indegree and outdegree of the
node, then select the other ends for these edges via preferential 
attachment.
iv) Delete Node: Select a node uniformly at random and delete
it with its incident edges.
 
In our experiments, we measure the average update times (i.e.,
edge insertion time (EI), node insertion time (NI), edge deletion
time (ED) and node deletion time (ND)) during the lifetime of a
dynamic reachability index. We used three versions of \alg --
DG0, DG1 and DG2 correspond to \alg with no intervals ($k=0$), 1
interval ($k=1$), and 2 intervals ($k=2$) per node, respectively.
Note that DG0 maintains only the DAG graph without using any
interval labeling and answers queries by performing a search on
the DAG graph. In contrast, the basic DFS performs the query
directly on the input graph, since it obviously does not maintain
the DAG.


\begin{figure*}[!ht]
\centerline{
\subfigure[FrenchWiki]{
\includegraphics[width=1.35in,height=1.00in]{./daggerplots/frwiki_n7550000.tt-bw.eps}	
}
\subfigure[PatentCitation]{
\includegraphics[width=1.35in,height=1.00in]{./daggerplots/cit-Patents.txt.sorted.tt-bw.eps}	
}
\subfigure[ER1M]{
\includegraphics[width=1.35in,height=1.00in]{./daggerplots/er1Mk2.tt-bw.eps}	
}
\subfigure[BA1M]{
\includegraphics[width=1.35in,height=1.00in]{./daggerplots/ba1Mk2bidir.tt-bw.eps}	
}}
\vspace{-0.15in}
\caption{\small Total time comparison on dynamic datasets}
\vspace{-0.1in}
\label{fig:dynamictotal}
\end{figure*}

\begin{table}[!ht]
\centering
\small
\subtable[Real Graphs]{
\begin{tabular}{|l||ccccc||cc|}
\hline
Data & \multicolumn{5}{|c||}{FrenchWiki} & \multicolumn{2}{|c|}{Citation}\\
\hline
Method & Q & EI & ED & NI & ND & Q & NI\\
\hline
DFS & 410 & - & - & - & - & 0.19 & - \\
DG0 & 221 & 60 & 253 & 0.06 & 191 & 0.31 & 0.06 \\
DG1 & 148 & 48 & 267 & 0.02 & 189 & 0.10 & 0.06 \\
DG2 & 128 & 62 & 279 & 0.02 & 192 & 0.08 & 0.06 \\
\hline
\end{tabular}
}
%\caption{\small Average Operation Times (in ms) on Real Data}
%\end{table}
%\vspace{0.2in}
%\begin{table*}
%\hspace{-0.4in}
\scriptsize
\subtable[Synthetic Graphs]{
\begin{tabular}{|l||ccccc||ccccc|}
\hline
Data & \multicolumn{5}{|c||}{ER1M} & \multicolumn{5}{|c|}{BA1M}\\
\hline
 & Q & EI & ED & NI & ND & Q & EI & ED & NI & ND\\
\hline
DFS & 311 & - & - & - & - & 448 & - & - & - & -  \\
DG0 & 119 & 212 & 775 & 0.01 & 538  & 75 & 172 & 2032 & 0.03 & 2726\\
DG1 & 46 & 203 & 832 & 0.13 & 548  & 39 & 148 & 2138 & 0.13 & 2769\\
DG2 & 44 & 319 & 871 & 0.10 & 562 & 38 & 218 & 2202 & 0.07 & 2804 \\
\hline
\end{tabular}
}
\vspace{-0.2in}
\caption{\small Average Operation Times (in ms) on Real and
Synthetic Data. $Q$ refers to query time, $EI$ and $ED$ to edge
insertion and deletion, and $NI$ and $ND$ to node insertion and
deletion.}
\vspace{-0.2in}
\label{tab:dynamicresults}
\end{table}

\subsection{Results}

In Figure~\ref{fig:dynamictotal}, we plot the total time taken to
perform all the operations (updates and queries) for DFS and 
the \alg variants DG0,
DG1, and DG2. The total time (in sec) is plotted against the
number of reachability queries per update operation. DAGGER has the
advantage of fast querying at the cost of index maintenance,
whereas DFS has no update cost. These plots make it clear that 
DG1 amortizes the maintenance costs as long as there are 
2-4 queries per update operation, which is quite reasonable
for an online system. The average update and query times on 
each of the graph datasets are shown in
Tables~{\ref{tab:dynamicresults}(a)} and {\ref{tab:dynamicresults}(b)}.
We discuss dataset specific results below.

\textbf{FrenchWiki:} In Figure~\ref{fig:dynamictotal}(a),
we see that DG0 performs better DFS in total time starting with 
4 queries per update. 
In other words, the efficient dynamic DAG/SCC maintenance in \alg
is enough to outperform the baseline DFS method.
On the other hand, the interval labeling and maintenance in \alg
offers even more significant benefits.
We can observe that 
\alg with interval labeling is better than DFS after just
2 queries per update. 
However, it is interesting to note that there is no big 
difference in the performance of DG1 and DG2. That is, using two
interval labels does not improve the total time. 
In Table~{\ref{tab:dynamicresults}(a)} we can see that whereas the
average query time is indeed better for DG2, unfortunately it
incurs more overhead for the update operations due to the
extra cost of maintaining one more interval, in particular for
edge insertion/deletion.


\textbf{PatentCitation:} In this dataset the only update
operation is node insertion with outgoing edges. From
Table~{\ref{tab:dynamicresults}(a)} we observe that the cost of node
insertions are very close for all versions of DAGGER due to the
fact that there is no DAG maintenance (e.g., input graph is
always a DAG) and no label propagation. Therefore, the plot in
Figure~\ref{fig:dynamictotal}(b) reflects mainly the query time of
the methods. DG0 has worse query times than DFS, even though it
performs the same search as DFS, which can be attributed to the
overhead of the \alg graph.  However, dynamic interval labeling
provides a significant improvement on querying performance, with
two intervals (DG2) providing better query times than a single
interval label per node (DG1).

\textbf{ER1M: } Table~\ref{tab:dynamicdata} shows that this graph
has a large connected component one-third the size of the input
graph; almost all the remaining nodes are single node components.
Table~{\ref{tab:dynamicresults}(b)} shows the break down in terms of
average operation times.  We observe that DFS querying is three
times slower than even DG0! Further, dynamic interval labeling
helps, but the small query performance gain obtained by utilizing
two intervals per node instead of single interval does not pay
off the label maintenance cost. In particular, edge insertion
with DG2 is significantly slower than DG1, because when the
interval of the huge component is enlarged, this change has to be
propagated up for all the incoming edges of the huge component,
and there can be many such incoming edges.  However, the cost of
edge insertion does not increase when moving from DG0 to DG1,
because interval labels also provide pruning when updating the
DAG. The plot in Figure~\ref{fig:dynamictotal}(c) shows that DG1 is
the best method overall, and all \alg variants are preferable to
DFS, if there are at least 2 queries per update.

\textbf{BA1M: } The results are similar to those
for ER1M (see Table~{\ref{tab:dynamicresults}(b)}).
The main difference is that BA1M has a much larger SCC,
which reduces the size of the DAG significantly. Hence,
there is a greater performance difference between DFS and
\alg methods as seen in Figure~\ref{fig:dynamictotal}(e). DG1
outperforms DFS starting with 2 queries per update.

In summary, over all the real and synthetic datasets, we observe
that typically DG1 gives the best overall performance, whereas
even DG0 (i.e., just maintaining the strongly connected
components without labeling) results in a significant improvement
over DFS. 
%The cost of update operations with \alg are in the order of the
%cost of querying with DFS, therefore the index amortizes the
%maintenance cost if it receives at least a few queries per
%update operation..  
As expected, \alg amortizes the index maintenance cost against
query times, and thus the more the queries received, the more the
benefit.  It is also interesting to note that a single interval
label provides the best performance, and going to two labels does
not confer any effective advantage.  There are two reasons for
this: i) when the DAG corresponding to the input graph is very
sparse (or tree-like), a single interval is sufficient to provide
fast querying, since it captures most of the topology, and ii)
dynamically updating labels makes the labels less random, since
our current label propagation algorithm is deterministic, and of
course there is extra cost associated with label propagation.


